SOEN-101: Code Generation by Emulating Software Process Models Using Large Language Model Agents

Software process models are essential to facilitate collaboration and communication among software teams to solve complex development tasks. Inspired by these software engineering practices, we present FlowGen - a code generation framework that emulates software process models based on multiple Large Language Model (LLM) agents. We emulate three process models, FlowGenWaterfall, FlowGenTDD, and FlowGenScrum, by assigning LLM agents to embody roles (i.e., requirement engineer, architect, developer, tester, and scrum master) that correspond to everyday development activities and organize their communication patterns. The agents work collaboratively using chain-of-thought and prompt composition with continuous self-refinement to improve the code quality. We use GPT3.5 as our underlying LLM and several baselines (RawGPT, CodeT, Reflexion) to evaluate code generation on four benchmarks: HumanEval, HumanEval-ET, MBPP, and MBPP-ET. Our findings show that FlowGenScrum excels compared to other process models, achieving a Pass@1 of 75.2, 65.5, 82.5, and 56.7 in HumanEval, HumanEval-ET, MBPP, and MBPP-ET, respectively (an average of 15% improvement over RawGPT). Compared with other state-of-the-art techniques, FlowGenScrum achieves a higher Pass@1 in MBPP compared to CodeT, with both outperforming Reflexion. Notably, integrating CodeT into FlowGenScrum resulted in statistically significant improvements, achieving the highest Pass@1 scores. Our analysis also reveals that the development activities impacted code smell and exception handling differently, with design and code review adding more exception handling and reducing code smells. Finally, FlowGen models maintain stable Pass@1 scores across GPT3.5 versions and temperature values, highlighting the effectiveness of software process models in enhancing the quality and stability of LLM-generated code.

==> Section/Motivation.tex <==
\peter{this section should be merged with intro}
\feng{this part already merged with intro}

% \section{Motivation}
% The inception of Large Language Models (LLMs), such as ChatGPT, has significantly eased software development from commit message generation~\cite{zhang2024automatic}, merge-conflict resolution~\cite{shen2023git}, and method renaming~\cite{alomar2024refactor}. Despite their advances, LLMs face two major challenges: (1) \textbf{\textit{Explicit Knowledge Transfer during Model Training}:} Before deployment into real-world development, LLM may need to be fine-tuned with high-quality data, additional data, and domain-specific target data~\cite{lin2024dataefficient}. (2) \textbf{\textit{Prompt Engineering}:} Involves engineering queries that aid in obtaining superior results from the LLM. For instance, adding personalization to the LLM, such as identifying yourself as a ``domain expert" in the ``X" field, can enhance the quality of the LLM response~\cite{white2023chatgpt,shao2023characterllm}. (3) Other methodologies, like Few-Shot~\cite{kumar2021reordering} and In-Context Learning~\cite{yao2023samples}, also prove to be beneficial.

% Recently, agent-based LLM has garnered the most attention. Similar to the concept of adding personalization, these agents are LLMs that can be customized to carry out specific tasks. For example, an agent can be designed to act as a code reviewer or tester. As shown in Copilot~\cite{bird2022taking}, such agents can be integrated into the software development life-cycle involving real developers to streamline different programming tasks(e.g., Code-Review, helping developers become more productive). However, the novelty lies in using multiple LLM agents, each specialized in different domains, to collaborate and solve complex tasks. For example, ~\citet{yang2023autogpt} showed how high-level tasks can be broken down into multi-step tasks to help solve complex problems. Our study is highly inspired by these collaborative agent-based approaches, with a focus on Flow Engineering~\cite{ridnik2024code}, which shows how multi-step LLM agent interaction and reasoning can influence LLMs' performance on Code Generation tasks. 

% In real-world development, building software involves substantial effort and communication. To ensure software robustness, software teams often adhere to a software process model, tailoring their approach to the software type and team size. For safety-critical software, a waterfall model might be followed, while smaller startups emphasizing rapid prototyping may opt for Scrum. To the best of our knowledge, the most popular software process models are \water, \tdd, and \scrum. 

% Although different software process models are considered to be advantageous for different systems, their impact on code generation tasks remains unknown. Earlier research by~\citet{qian2023communicative} has adopted the \water model within LLM to develop fully agent-assisted software. Yet, this work did not specifically focus on the software process model itself.~\citet{xu2023exploring} also showed that LLM could give different responses according to personalized roles. Inspired by these works, we present a novel adaptation of flow engineering on software process models in real-world development. We aim to study how different process models influence the LLM's code generation capability. Specifically, we investigate whether process models improve LLM interaction and reasoning, contributing to enhancing code generation. 

% Our study yields several practical relevance. Firstly, aligning these process models with the software development cycle adheres closely to real industry standards. This compatibility ensures that each role within these models can be interchanged with human counterparts, which enhances the adoption of our research findings to real-world applications. Moreover, we perform the first in-depth study on how interactions amongst LLM agents can improve code generation, which provides valuable insight for further research in diverse problem domains.

==> Section/RelatedWork.tex <==
% \section{Related Works}
% Inspired by Agent-Based research, our focus is on 
% employing LLM agents to implement software process models and conducting code generation task. We categorize the related work into two main groups: 

% \subsection{Code Generation}
% Code generation stands as an active research area, marked by numerous on-going efforts to improve LLM capabilities for producing high-quality code. For example, ~\citet{zhou2023language} introduced a Language Agent Tree Search algorithm, 
%  ~\citet{wei2023chainofthought} introduced chain-of-Thought Prompting, \citet{li2023structured} introduced Structured Chain-of-Thought Prompting, ~\citet{shinn2023reflexion} introduced a reinforcement learning mechanism. These works attempts to improve the behavior of the LLM by integrating novel training algorithms.
 
% Other works utilize software process models for the LLM. For example, ~\citet{hong2023metagpt} and ~\citet{qian2023communicative} use WaterFall model to generate a project code based on a single user requirement. However, these studies do not delve into the software process model itself and how different component within it contribute to improved reasoning and code generations. There is also the work by~\citet{dong2023selfcollaboration} also builds a virtual software team with three roles(Analyst/Coder/Tester) in such software teams, which is not very similar to the real-world development, and skips some of the roles' tasks in the software process models. Specifically, an analyst not only writes an analysis report in a real team but also takes part in the test cases meeting and gives suggestions to the tester to revise their test cases.

% In comparison, we focus on the popular software process models that are used in real-world development and study how these stages and roles affect performance. Some parts of the experiments are similar to these priors, but due to the environment settings(model-versions, temperature, prompt templates, etc.), the experiments are not the same as these priors' papers.

% \subsection{Agent-Based}

% Recently, some interesting experiments have used LLMs to build a virtual team to complete different kinds of tasks, which is also called Agent-Based. 

% ~\citet{park2023generative}, they built 25 virtual characters, each controlled by the LLM-powered agent. These agents live and interact in a sandbox environment, with emergent social behaviors: one agent wants to throw a party, then it autonomously spreads invitations to the party, and it can even ask each other about the dates and coordinate for the right time. Such an experiment shows LLMs may have the ability to break a requirement into a task list and finish the tasks.

% ~\citet{xu2023exploring} also built a virtual team to play communication games: Werewolf. They ask each agent to play different roles in a game, during the part of question-answering, they need to reflect based on their role and generate reasonable responses. Such an experiment shows LLMs may have the ability to communicate with each other based on their specific roles.
